MS-DARTS: Mean-Shift Based Differentiable Architecture Search

Differentiable Architecture Search (DARTS) is an effective continuous relaxation-based network architecture search (NAS) method with low search cost. It has attracted significant attentions in Auto-ML research and becomes one of the most useful paradigms in NAS. Although DARTS can produce superior efficiency over traditional NAS approaches with better control of complex parameters, oftentimes it suffers from stabilization issues in producing deteriorating architectures when discretizing the continuous architecture. We observed considerable loss of validity causing dramatic decline in performance at this final discretization step of DARTS. To address this issue, we propose a Mean-Shift based DARTS (MS-DARTS) to improve stability based on sampling and perturbation. Our approach can improve bot the stability and accuracy of DARTS, by smoothing the loss landscape and sampling architecture parameters within a suitable bandwidth. We investigate the convergence of our mean-shift approach, together with the effects of bandwidth selection that affects stability and accuracy. Evaluations performed on CIFAR-10, CIFAR-100, and ImageNet show that MS-DARTS archives higher performance over other state-of-the-art NAS methods with reduced search cost.

==> tmp.tex <==
Eq.\eqref{eq:zela:alpha} solves the robust optimization problem \cite{chen2020stabilizing} minimizing the worst-case loss around a neighborhood of an architecture $\boldsymbol{A}$. In fact, at each sampled iteration, $W$ is re-estimated by changing the original architecture only once. However, this cannot provide enough a solution to flat the loss landscape of $\mathcal{L}_{train}$, which is crucial for stability control. In comparison, we propose MS-DARTS, the recursive update of the architecture $\boldsymbol{A}$ with the mean-shift algorithm in Eq.\eqref{eq:zela:alpha} before minimizing $\mathcal{L}_{train}$ can effectively smooth the landscape, such that better accuracy and stability can be obtained. One additional advantage of this recursive updating of $\boldsymbol{A}$ is efficiency, since less iterations are needed to find $W$ by minimizing $\mathcal{L}_{train}$. In addition, MS-DARTS also can address the flatness of minima. During training, flatter minima \cite{FlatMinima}, and thus better stability in architecture performance.


% -------------------------------
Eq.\eqref{eq:zela:alpha}, the best weight $\overline{W}$ is estimated by searching $A$ with the worst case around a neighborhood of the original architecture. Thus, the flattening of the architectural search landscape by recursively forcing the original architecture to move toward a smooth region can improve the weight estimation.  Eq.\eqref{eq:delta:update:alpha} can achieve more smoothing effect and lead to good stability in DARTS in comparison to Eq.\eqref{eq:zela:alpha}. 
Finally, the movements in Eq.\eqref{eq:delta:update:alpha} do not involve any optimization on $\overline{W}$. 
Thus, less iterations are needed to optimize the weights and thus better efficiency can be achieved.   
